MTevent: A Multi-Task Event Camera Dataset for 6D Pose Estimation and Moving Object Detection

Mobile robots are reaching unprecedented speeds, with platforms like Unitree B2, and Fraunhofer O3dyn achieving maximum speeds between 5 and 10 m/s. However, effectively utilizing such speeds remains a challenge due to the limitations of RGB cameras, which suffer from motion blur and fail to provide real-time responsiveness. Event cameras, with their asynchronous operation, and low-latency sensing, offer a promising alternative for high-speed robotic perception. In this work, we introduce MTevent, a dataset designed for 6D pose estimation and moving object detection in highly dynamic environments with large detection distances. Our setup consists of a stereo-event camera and an RGB camera, capturing 75 scenes, each on average 16 seconds, and featuring 16 unique objects under challenging conditions such as extreme viewing angles, varying lighting, and occlusions. MTevent is the first dataset to combine high-speed motion, long-range perception, and real-world object interactions, making it a valuable resource for advancing event-based vision in robotics. To establish a baseline, we evaluate the task of 6D pose estimation using NVIDIA's FoundationPose on RGB images, achieving an Average Recall of 0.22 with ground-truth masks, highlighting the limitations of RGB-based approaches in such dynamic settings. With MTevent, we provide a novel resource to improve perception models and foster further research in high-speed robotic vision. The dataset is available for download https://huggingface.co/datasets/anas-gouda/MTevent

==> Tables/comparison.tex <==

\begin{table*}[!ht]
    \centering
    \caption{Comparison of datasets acquired using an event camera in an indoor environment. Event6D records scenes in a warehouse setting with varying degrees of freedom. The objects are larger than typical household objects, measuring from $19\times42\times32$~cm to $80\times120\times14$~cm.}
    \renewcommand{\arraystretch}{1.3} % Increase row height for better readability
    \setlength{\tabcolsep}{10pt} % Adjust column spacing
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l l l c c c l}  
        \toprule
        \textbf{Dataset} & \textbf{Environment} & \makecell{\textbf{Independently} \\ \textbf{Moving Objects (IMO)}} & \makecell{\textbf{Suitable for} \\ \textbf{Mobile Robotics}} & \textbf{IMO Pose} & \makecell{\textbf{Distance} \\ \textbf{to Objects}} & \textbf{Ground Truth} \\ 
        \midrule
        M3ED\cite{chaney2023m3ed}   & Indoor + Outdoor & Pedestrians, Cars & \xmark & \cmark & Large  & Lidar + RTK \\  
        EViMO2\cite{evimo2} & Indoor           & Household Objects & \xmark & \cmark & Small  & MoCAP \\  
        EDAT24\cite{duarte2024event} & Indoor           & Small Manufacturing Objects & \xmark & N/A & Small & N/A \\  
        VECtor\cite{gao2022vector} & Indoor           & None               & \xmark & N/A & N/A & MoCAP + ICP \\  
        DSEC \cite{dsec}  & Indoor + Outdoor & Pedestrians, Cars & \xmark & \xmark & Large  & Motion Capture + GPS \\  
        EED \cite{eed}   & Indoor           & UAVs               & \xmark & \xmark & N/A & Manual \\  
        E-Pose \cite{epose}   & Indoor           & Objects are Static               & \xmark & \xmark & Small & ZED Mini Camera \\  
        Event6D (ours) & Indoor          & 16 Objects (Fig.~\ref{fig:ECMR_objects}) & \cmark & \cmark & Varying & Motion Capture \\  
        \bottomrule
    \end{tabular}%
    }
    
    \label{tab:comparison}
\end{table*}


==> figures/objects_orig.tex <==
\begin{figure*}

    \centering
    % Top row with 8 images
    \begin{minipage}{0.35\textwidth} % Adjusting the width of each subfigure
        \centering        \includegraphics[width=4.5cm,height=4.5cm,keepaspectratio]{images/objects/obj_000001.jpg}  
         \\[-0.1cm]
    \end{minipage}    
    \begin{minipage}{0.12\textwidth}
        \centering        \includegraphics[width=\textwidth,height=2cm,keepaspectratio]{images/objects/obj_000002.jpg}
    \end{minipage}    
    \begin{minipage}{0.15\textwidth}
        \centering        \includegraphics[width=\textwidth,height=2cm,keepaspectratio]{images/objects/obj_000003.jpg}
        
    \end{minipage}    
    \begin{minipage}{0.11\textwidth}
        \centering      \reflectbox{  \includegraphics[width=\textwidth,height=2cm,keepaspectratio]{images/objects/obj_000004.jpg}}
        
    \end{minipage}    
    \begin{minipage}{0.14\textwidth}
        \centering        \includegraphics[width=\textwidth,height=2cm,keepaspectratio]{images/objects/obj_000005.jpg}
    \end{minipage}
    \\[-0.30cm]
    
    \begin{minipage}{0.10\textwidth}
        \centering      
        \includegraphics[width=2.1cm,height=2.1cm]{images/objects/obj_000006.jpg}
    \end{minipage}
    \begin{minipage}{0.14\textwidth}
        \centering       \reflectbox{ \includegraphics[width=3.4cm,height=3.4cm,keepaspectratio]{images/objects/obj_000007.jpg}}
    \end{minipage}
    \begin{minipage}{0.18\textwidth}
        \centering
        \includegraphics[width=3.1cm,height=2.6cm,keepaspectratio]{images/objects/obj_000008.jpg}
    \end{minipage}
    % Bottom row with 8 images
    \begin{minipage}{0.12\textwidth}
        \centering        \includegraphics[width=\textwidth,height=2cm,keepaspectratio]{images/objects/obj_000009.jpg}
    \end{minipage}
    \begin{minipage}{0.12\textwidth}
        \centering        \includegraphics[width=\textwidth,height=2cm,keepaspectratio]{images/objects/obj_000010.jpg}
    \end{minipage}
    \begin{minipage}{0.15\textwidth}
        \centering        \includegraphics[width=2.4cm,height=2.4cm,keepaspectratio]{images/objects/obj_000011.jpg}
    \end{minipage}
    \\[-0.5cm]
    
    \begin{minipage}{0.15\textwidth}
        \centering        \includegraphics[width=2cm,height=2cm,keepaspectratio]{images/objects/obj_000012.jpg}
    \end{minipage}
    \begin{minipage}{0.13\textwidth}
        \centering
        \includegraphics[width=\textwidth,height=1.8cm,keepaspectratio]{images/objects/obj_000013.jpg}
    \end{minipage}
    \begin{minipage}{0.26\textwidth}
        \centering
    \includegraphics[width=3.3cm,height=2.9cm]{images/objects/obj_000014.jpg}
    \end{minipage}
    \begin{minipage}{0.26\textwidth}
        \centering
        \includegraphics[width=3.8cm,height=2.5cm,trim=0 0 30 0, clip]{images/objects/obj_000015.jpg}
    \end{minipage}
    \begin{minipage}{0.11\textwidth}
        \centering 
        \reflectbox{\includegraphics[width=\textwidth,height=2cm,keepaspectratio,  trim=0 0 10 0, clip]{images/objects/obj_000016.jpg}}
    \end{minipage}
    \caption{The figure illustrates the Event6D dataset objects. The first row displays four industrial objects, including the Euro pallet and three different Euro containers. The last object in the first row is an Amazon Basics suitcase. The second and third rows showcase IKEA storage objects, which are widely available and standardized. Event6D features a diverse selection of objects, balancing industrial relevance with real-world variety, to support 3D bounding box detection and 6D pose estimation for moving objects. The objects are sequentially assigned unique IDs from 1 to 16, starting from the top-left and proceeding row-wise.
    }
    \label{fig:ECMR_objects}
\end{figure*}



==> sec/10_comments.tex <==
\begin{comment}
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.


\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}


This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.
\end{comment}

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
